Optimal Regret Bounds for Collaborative Learning in Bandits

We consider regret minimization in a general collaborative multi-agent multi-armed bandit model, in which each agent faces a finite set of arms and may communicate with other agents through a central controller. The optimal arm for each agent in this model is the arm with the largest expected mixed reward, where the mixed reward of each arm is a weighted average of its rewards across all agents, making communication among agents crucial. While near-optimal sample complexities for best arm identification are known under this collaborative model, the question of optimal regret remains open. In this work, we address this problem and propose the first algorithm with order optimal regret bounds under this collaborative bandit model. Furthermore, we show that only a small constant number of expected communication rounds is needed.

==> author_response.tex <==
% \documentclass[11pt]{article}
% \usepackage[margin=0.85in,letterpaper]{geometry}
% \usepackage{lineno}
% \linenumbers
% \usepackage{color}
% \usepackage{xcolor}
% \usepackage{amssymb,graphicx}

% \begin{document}
% % author response goes here; maximum 1 page, including any references
% \paragraph{Reviewer $2$:}{We appreciate your positive feedback. We are glad that the paper's quality and the novelty of our algorithm were well-received. 
% In response to your comment on the analysis, we agree that our approach includes standard techniques from the bandit literature, like confidence intervals. However, due to mixing samples from different agents, the standard Chernoff-Hoeffding type inequalities cannot be directly applied, and the confidence intervals are achieved using a mixture of martingales approach. Our analysis also introduces novel aspects, such as using $1-1/\log(t)$ confidence intervals compared to the standard $1-1/t$, and projections to the $(1/\log(\log(t))$, $\log(\log(t)))$ interval. These elements are required to analyze a carefully crafted algorithm designed to address an existing gap in the literature. We will emphasize these points in the final version.}
% \paragraph{Reviewer $5$:}{Thank you for your comprehensive review and for recognizing the interest in collaborative learning across several applications. 
% We here address your comments in the weaknesses section, hoping to positively impact your evaluation.
% \textcolor{blue}{\bf 1.} The simplicity of the problem post-solution belies its initial complexity. To underscore the novelty's significance, we refer to Réda et al., (2022), a NeurIPS 2022 Oral presentation, highlighting the challenge of designing algorithms with order-optimal regret bounds in this setting.
% %This is notably mentioned 
% In their Section 5 concluding remarks, this challenging problem is considered an ``interesting subsequent work''. Also, the order-optimal regret bounds remained open even in simpler settings, a special case in Shi et al., (2021). \textcolor{blue}{\bf 2.} Our results address the asymptotic regret bounds. We also provide a finite time analysis that shows an ``order-optimal'' regret bound albeit with possibly large constants. We will further clarify this point. \textcolor{blue}{\bf 3.} Regarding communication, we follow the literature: Hillel et al. (2013); Karpov et al. (2020); Chen et al. (2021); Zhu et al. (2021) and, Shi et al., 2021, Réda et al., 2022. 
% As to the possibility of improving the bound with increased communication, the answer is negative. The reason is that we already achieved the order-optimal regret bound with a small constant number of communication rounds. Note that in the statement of lower bound in Lemma~1 the agents are allowed to communicate at each round. In Theorem~5, we prove a matching upper bound on regret with a small constant number of communication rounds. Given the lower bound, this cannot be improved even by increased communication. 
% \textcolor{blue}{$\Diamond$} We regret any difficulties you faced in reading the paper. Switching to $\pi’$ is detailed at the bottom of page 7 in the paragraph starting with \textbf{Exploitation/Switching to $\pi’$}. To enhance clarity, we will transform this section into a subsection and reference it in Algorithm 1. The choice of $\pi’$ is also specified in Theorem 5 where the result is stated. 
% \textcolor{blue}{$\Diamond$} Positioning our results within the context of existing literature is vital, especially as we address unresolved problems from Shi et al., (2021), and Réda et al., (2022). Following your suggestion, we will move our main result statement earlier in the introduction.
% }

% \paragraph{Reviewer $6$:}{Thank you for your positive feedback. We here address your comments and hope to further improve your evaluation of our work.
% Regarding the regret bound, which is a focal point of your comments, we acknowledge that our bound is an order-optimal, problem-dependent, asymptotic regret bound. As we provide a finite time analysis, our bound is order optimal, albeit with large constants. We appreciate your suggestion and will emphasize these points more explicitly in the final version. We will also modify the term ``Optimal'' in the title to ``Order-Optimal'' as per your recommendation. 
% \textcolor{blue}{\bf 1.} We agree. However, this is an additive term that is dominated by the leading term. \textcolor{blue}{\bf 2.} We acknowledge that the constant factors are possibly large. \textcolor{blue}{\bf 3.} We acknowledge this point; $T_0$ can also be understood as an additive term in regret.
% \textcolor{blue}{$\Diamond$}~We used the approximate notation following Réda et al., (2022) and Kaufmann and Koolen (2021), for simplicity, without compromising the rigor of our statements. In light of your feedback, we will revise this to use rigorous inequalities to enhance clarity. \textcolor{blue}{$\Diamond$} Regarding the proof hints, we are grateful for your suggestions. We will incorporate a recall of $g_M$, $\tau_1$, and $\delta$ in Equation~(30) and will add similar enhancements to the proofs where applicable.
% \textcolor{blue}{$\Diamond$} Finally, we thank you for your detailed and thoughtful minor comments. All these points will be carefully accommodated in the final version.
% }

% \end{document}
